Acoustic Characterization of Environments (ACE) Challenge Results Technical Report

This document provides the results of the tests of acoustic parameter estimation algorithms on the Acoustic Characterization of Environments (ACE) Challenge Evaluation dataset which were subsequently submitted and written up into papers for the Proceedings of the ACE Challenge. This document is supporting material for a forthcoming journal paper on the ACE Challenge which will provide further analysis of the results.

==> ana_eval_gt_partic_results_combined_Phase3_TR_P3S_DRR_dB_-1dB_SNR_All_Noises_sub_ICASSP_2015_DRR_2-ch_Gerkmann_NR_FFT_subband_cite_bias_sub.tex <==
 1 & 25.12 & -11.07 & 124.4 & 0 \\ 
\hline
 2 & 31.62 & -9.93 & 100.8 & 0 \\ 
\hline
 3 & 39.81 & -11.69 & 138.1 & 0 \\ 
\hline
 4 & 50.12 & -11.55 & 135.4 & 0 \\ 
\hline
 5 & 63.10 & -14.82 & 221.5 & 0 \\ 
\hline
 6 & 79.43 & -16.09 & 260.6 & 0 \\ 
\hline
 7 & 100.00 & -16.18 & 262.6 & 0 \\ 
\hline
 8 & 125.89 & -17.74 & 318.4 & 0 \\ 
\hline
 9 & 158.49 & -16.76 & 283.2 & 0 \\ 
\hline
10 & 199.53 & -16.71 & 282.4 & 0.07086 \\ 
\hline
11 & 251.19 & -17.55 & 320 & -0.04596 \\ 
\hline
12 & 316.23 & -19.86 & 406.8 & 0.02029 \\ 
\hline
13 & 398.11 & -19.88 & 446.6 & -0.03424 \\ 
\hline
14 & 501.19 & -18.58 & 407.5 & 0.2808 \\ 
\hline
15 & 630.96 & -19.22 & 422.9 & 0.4172 \\ 
\hline
16 & 794.33 & -18.98 & 411.7 & 0.2086 \\ 
\hline
17 & 1000.00 & -18.26 & 397.9 & 0.3138 \\ 
\hline
18 & 1258.93 & -16.51 & 342 & 0.3056 \\ 
\hline
19 & 1584.89 & -13.69 & 273.6 & 0.1804 \\ 
\hline
20 & 1995.26 & -12.16 & 221.3 & 0.2725 \\ 
\hline
21 & 2511.89 & -9.824 & 161.2 & 0.4263 \\ 
\hline
22 & 3162.28 & -8.763 & 116.2 & 0.0871 \\ 
\hline
23 & 3981.07 & -8.229 & 98.17 & 0.03782 \\ 
\hline
24 & 5011.87 & -7.944 & 105 & 0.1668 \\ 
\hline
25 & 6309.57 & -11.33 & 217.6 & -0.1192 \\ 
\hline
26 & 7943.28 & -11.28 & 181.3 & 0.4844 \\ 
\hline


==> ana_eval_gt_partic_results_combined_Phase3_TR_P3S_DRR_dB_-1dB_SNR_All_Noises_sub_ICASSP_2015_DRR_2-ch_Gerkmann_NR_filtered_subband_cite_bias_sub.tex <==
 1 & 25.12 & 1.549 & 55.03 & -0.08924 \\ 
\hline
 2 & 31.62 & 2.725 & 55.21 & -0.02208 \\ 
\hline
 3 & 39.81 & 1.071 & 45.23 & -0.01651 \\ 
\hline
 4 & 50.12 & 1.472 & 49.75 & -0.07177 \\ 
\hline
 5 & 63.10 & -1.68 & 46.52 & 0.02834 \\ 
\hline
 6 & 79.43 & -3.424 & 73.13 & -0.05226 \\ 
\hline
 7 & 100.00 & -3.718 & 54.08 & 0.01433 \\ 
\hline
 8 & 125.89 & -5.129 & 69.49 & -0.01673 \\ 
\hline
 9 & 158.49 & -3.973 & 64.39 & -0.01465 \\ 
\hline
10 & 199.53 & -3.691 & 57.38 & -0.07436 \\ 
\hline
11 & 251.19 & -4.973 & 78.93 & -0.08322 \\ 
\hline
12 & 316.23 & -4.185 & 81.75 & -0.03248 \\ 
\hline
13 & 398.11 & -5.889 & 100.6 & -0.03229 \\ 
\hline
14 & 501.19 & -2.468 & 60.56 & -0.0483 \\ 
\hline
15 & 630.96 & 4.976 & 59.22 & 0.2309 \\ 
\hline
16 & 794.33 & 3.958 & 74.22 & 0.06978 \\ 
\hline
17 & 1000.00 & 1.334 & 66.66 & 0.04725 \\ 
\hline
18 & 1258.93 & 4.763 & 85.8 & 0.05723 \\ 
\hline
19 & 1584.89 & 3.613 & 97.12 & -0.01468 \\ 
\hline
20 & 1995.26 & -1.428 & 67.39 & 0.1753 \\ 
\hline
21 & 2511.89 & -3.336 & 69.66 & 0.1776 \\ 
\hline
22 & 3162.28 & -5.434 & 81.86 & 0.1788 \\ 
\hline
23 & 3981.07 & -5.05 & 58.64 & 0.1292 \\ 
\hline
24 & 5011.87 & -5.184 & 52.04 & 0.307 \\ 
\hline
25 & 6309.57 & -6.044 & 58.69 & 0.423 \\ 
\hline
26 & 7943.28 & -8.21 & 97.19 & 0.3824 \\ 
\hline


==> ana_eval_gt_partic_results_combined_Phase3_TR_P3S_DRR_dB_-1dB_SNR_All_Noises_sub_Velocity_cite_bias_sub.tex <==
 1 & 25.12 & 6.666 & 71.27 & -0.3122 \\ 
\hline
 2 & 31.62 & 7.271 & 77.33 & -0.2345 \\ 
\hline
 3 & 39.81 & 5.796 & 52.95 & 0.4081 \\ 
\hline
 4 & 50.12 & 4.112 & 47.97 & -0.5387 \\ 
\hline
 5 & 63.10 & 0.8308 & 25.3 & -0.03381 \\ 
\hline
 6 & 79.43 & -0.849 & 15.98 & 0.2145 \\ 
\hline
 7 & 100.00 & -0.7482 & 12.84 & 0.2447 \\ 
\hline
 8 & 125.89 & -1.524 & 18.11 & -0.01732 \\ 
\hline
 9 & 158.49 & -0.6441 & 12.47 & 0.2389 \\ 
\hline
10 & 199.53 & 1.399 & 12.16 & 0.3035 \\ 
\hline
11 & 251.19 & 0.3195 & 11.28 & 0.2986 \\ 
\hline
12 & 316.23 & -0.1609 & 14.97 & -0.007155 \\ 
\hline
13 & 398.11 & -0.2544 & 13.1 & 0.4424 \\ 
\hline
14 & 501.19 & 0.4963 & 14.18 & 0.2365 \\ 
\hline
15 & 630.96 & 0.04323 & 13.21 & 0.5434 \\ 
\hline
16 & 794.33 & -2.375 & 17.92 & 0.5036 \\ 
\hline
17 & 1000.00 & -1.427 & 16.46 & 0.2552 \\ 
\hline
18 & 1258.93 & -0.424 & 12.73 & 0.378 \\ 
\hline
19 & 1584.89 & -1.484 & 12.55 & 0.111 \\ 
\hline
20 & 1995.26 & -1.519 & 11.97 & 0.4146 \\ 
\hline
21 & 2511.89 & -1.96 & 15.83 & 0.2275 \\ 
\hline
22 & 3162.28 & -4.258 & 35.12 & 0.1885 \\ 
\hline


==> ana_eval_gt_partic_results_combined_Phase3_TR_P3S_DRR_dB_12dB_SNR_All_Noises_sub_ICASSP_2015_DRR_2-ch_Gerkmann_NR_FFT_subband_cite_bias_sub.tex <==
 1 & 25.12 & -11.07 & 124.4 & 0 \\ 
\hline
 2 & 31.62 & -9.93 & 100.8 & 0 \\ 
\hline
 3 & 39.81 & -11.69 & 138.1 & 0 \\ 
\hline
 4 & 50.12 & -11.55 & 135.4 & 0 \\ 
\hline
 5 & 63.10 & -14.82 & 221.5 & 0 \\ 
\hline
 6 & 79.43 & -16.08 & 260.5 & 0.02471 \\ 
\hline
 7 & 100.00 & -16.18 & 262.5 & 0.01651 \\ 
\hline
 8 & 125.89 & -17.72 & 318 & 0.002983 \\ 
\hline
 9 & 158.49 & -16.66 & 281.4 & -0.001785 \\ 
\hline
10 & 199.53 & -14.38 & 238.4 & 0.2941 \\ 
\hline
11 & 251.19 & -12.8 & 230.1 & 0.1328 \\ 
\hline
12 & 316.23 & -14.21 & 271.8 & 0.2068 \\ 
\hline
13 & 398.11 & -8.763 & 173.2 & 0.2037 \\ 
\hline
14 & 501.19 & -10.07 & 198 & 0.3363 \\ 
\hline
15 & 630.96 & -14.32 & 296.9 & 0.4747 \\ 
\hline
16 & 794.33 & -12.86 & 256.3 & 0.3056 \\ 
\hline
17 & 1000.00 & -8.95 & 162.8 & 0.3516 \\ 
\hline
18 & 1258.93 & -8.607 & 138.6 & 0.2633 \\ 
\hline
19 & 1584.89 & -6.031 & 85.57 & 0.1436 \\ 
\hline
20 & 1995.26 & -5.263 & 49.94 & 0.3933 \\ 
\hline
21 & 2511.89 & -3.448 & 38.42 & 0.5582 \\ 
\hline
22 & 3162.28 & -5.864 & 70.64 & 0.07543 \\ 
\hline
23 & 3981.07 & -6.482 & 74.5 & 0.04092 \\ 
\hline
24 & 5011.87 & -5.768 & 92.63 & 0.2733 \\ 
\hline
25 & 6309.57 & -8.998 & 202.8 & -0.1311 \\ 
\hline
26 & 7943.28 & -8.996 & 158.5 & 0.5613 \\ 
\hline


==> ana_eval_gt_partic_results_combined_Phase3_TR_P3S_DRR_dB_12dB_SNR_All_Noises_sub_ICASSP_2015_DRR_2-ch_Gerkmann_NR_filtered_subband_cite_bias_sub.tex <==
 1 & 25.12 & 2.379 & 60.72 & -0.1078 \\ 
\hline
 2 & 31.62 & 3.585 & 65.18 & -0.06329 \\ 
\hline
 3 & 39.81 & 2.011 & 51.62 & 0.01668 \\ 
\hline
 4 & 50.12 & 2.864 & 62.3 & -0.1149 \\ 
\hline
 5 & 63.10 & 0.3794 & 47.56 & -0.03139 \\ 
\hline
 6 & 79.43 & -2.239 & 65.68 & -0.02001 \\ 
\hline
 7 & 100.00 & -2.307 & 51.01 & 0.02981 \\ 
\hline
 8 & 125.89 & -3.294 & 53.79 & -0.05119 \\ 
\hline
 9 & 158.49 & -2.904 & 55.53 & -0.04611 \\ 
\hline
10 & 199.53 & -1.499 & 48 & -0.07928 \\ 
\hline
11 & 251.19 & -1.744 & 76 & -0.1336 \\ 
\hline
12 & 316.23 & 2.268 & 126.8 & -0.03916 \\ 
\hline
13 & 398.11 & 3.01 & 108.4 & -0.06728 \\ 
\hline
14 & 501.19 & 9.663 & 130.5 & -0.04887 \\ 
\hline
15 & 630.96 & 15.33 & 251 & 0.3112 \\ 
\hline
16 & 794.33 & 13.98 & 222.2 & 0.1411 \\ 
\hline
17 & 1000.00 & 11.63 & 168.5 & 0.06189 \\ 
\hline
18 & 1258.93 & 13.28 & 205.1 & -0.02043 \\ 
\hline
19 & 1584.89 & 10.74 & 165.4 & -0.172 \\ 
\hline
20 & 1995.26 & 5.079 & 63.92 & 0.2002 \\ 
\hline
21 & 2511.89 & 3.726 & 49.07 & 0.19 \\ 
\hline
22 & 3162.28 & 1.168 & 21.74 & 0.2083 \\ 
\hline
23 & 3981.07 & -0.891 & 12.79 & 0.1987 \\ 
\hline
24 & 5011.87 & -2.132 & 13.95 & 0.5264 \\ 
\hline
25 & 6309.57 & -2.778 & 18.21 & 0.6313 \\ 
\hline
26 & 7943.28 & -4.637 & 41.47 & 0.5358 \\ 
\hline


==> ana_eval_gt_partic_results_combined_Phase3_TR_P3S_DRR_dB_12dB_SNR_All_Noises_sub_Velocity_cite_bias_sub.tex <==
 1 & 25.12 & 6.071 & 61.6 & -0.3206 \\ 
\hline
 2 & 31.62 & 6.472 & 63.38 & -0.248 \\ 
\hline
 3 & 39.81 & 4.847 & 39.08 & 0.3735 \\ 
\hline
 4 & 50.12 & 3.429 & 34.6 & -0.4292 \\ 
\hline
 5 & 63.10 & 1.267 & 22.19 & -0.05965 \\ 
\hline
 6 & 79.43 & 1.059 & 18.45 & 0.1446 \\ 
\hline
 7 & 100.00 & 1.633 & 27.52 & 0.07875 \\ 
\hline
 8 & 125.89 & 2.816 & 26.63 & 0.1579 \\ 
\hline
 9 & 158.49 & 3.437 & 22.49 & 0.329 \\ 
\hline
10 & 199.53 & 3.423 & 20.43 & 0.427 \\ 
\hline
11 & 251.19 & 1.932 & 10.2 & 0.4898 \\ 
\hline
12 & 316.23 & 2.389 & 13.97 & 0.1019 \\ 
\hline
13 & 398.11 & 1.549 & 11.21 & 0.5946 \\ 
\hline
14 & 501.19 & 1.917 & 13.42 & 0.4018 \\ 
\hline
15 & 630.96 & 1.58 & 9.898 & 0.7291 \\ 
\hline
16 & 794.33 & -0.7663 & 8.04 & 0.6722 \\ 
\hline
17 & 1000.00 & 0.3193 & 7.474 & 0.5171 \\ 
\hline
18 & 1258.93 & 1.064 & 7.895 & 0.5567 \\ 
\hline
19 & 1584.89 & -0.7871 & 9.227 & 0.1832 \\ 
\hline
20 & 1995.26 & -0.4783 & 7.107 & 0.5546 \\ 
\hline
21 & 2511.89 & -0.2629 & 5.645 & 0.4636 \\ 
\hline
22 & 3162.28 & -2.402 & 17.08 & 0.3028 \\ 
\hline


==> ana_eval_gt_partic_results_combined_Phase3_TR_P3S_DRR_dB_18dB_SNR_All_Noises_sub_ICASSP_2015_DRR_2-ch_Gerkmann_NR_FFT_subband_cite_bias_sub.tex <==
 1 & 25.12 & -11.07 & 124.4 & 0 \\ 
\hline
 2 & 31.62 & -9.93 & 100.8 & 0 \\ 
\hline
 3 & 39.81 & -11.69 & 138.1 & 0 \\ 
\hline
 4 & 50.12 & -11.55 & 135.4 & 0 \\ 
\hline
 5 & 63.10 & -14.82 & 221.5 & 0 \\ 
\hline
 6 & 79.43 & -16.04 & 259.7 & 0.05147 \\ 
\hline
 7 & 100.00 & -16.13 & 261.8 & 0.03538 \\ 
\hline
 8 & 125.89 & -17.57 & 315 & 0.01621 \\ 
\hline
 9 & 158.49 & -15.74 & 264.7 & -0.008995 \\ 
\hline
10 & 199.53 & -10.16 & 174.8 & 0.1689 \\ 
\hline
11 & 251.19 & -7.795 & 148.8 & 0.1611 \\ 
\hline
12 & 316.23 & -8.078 & 146.6 & 0.2706 \\ 
\hline
13 & 398.11 & -3.031 & 66.69 & 0.2798 \\ 
\hline
14 & 501.19 & -5.898 & 105.8 & 0.4782 \\ 
\hline
15 & 630.96 & -11.09 & 216.7 & 0.5535 \\ 
\hline
16 & 794.33 & -9.513 & 180.4 & 0.3579 \\ 
\hline
17 & 1000.00 & -5.003 & 74.8 & 0.3796 \\ 
\hline
18 & 1258.93 & -6.076 & 81.9 & 0.2277 \\ 
\hline
19 & 1584.89 & -4.768 & 61.04 & 0.1319 \\ 
\hline
20 & 1995.26 & -4.51 & 36.79 & 0.4406 \\ 
\hline
21 & 2511.89 & -2.379 & 23.53 & 0.6218 \\ 
\hline
22 & 3162.28 & -5.297 & 60.56 & 0.05556 \\ 
\hline
23 & 3981.07 & -6.315 & 73.16 & 0.03712 \\ 
\hline
24 & 5011.87 & -5.287 & 89.22 & 0.3047 \\ 
\hline
25 & 6309.57 & -8.592 & 202.7 & -0.1197 \\ 
\hline
26 & 7943.28 & -8.665 & 159.5 & 0.5803 \\ 
\hline


==> ana_eval_gt_partic_results_combined_Phase3_TR_P3S_DRR_dB_18dB_SNR_All_Noises_sub_ICASSP_2015_DRR_2-ch_Gerkmann_NR_filtered_subband_cite_bias_sub.tex <==
 1 & 25.12 & 3.173 & 66.39 & -0.05979 \\ 
\hline
 2 & 31.62 & 4.545 & 73.28 & 0.001786 \\ 
\hline
 3 & 39.81 & 3.271 & 61.48 & -0.01371 \\ 
\hline
 4 & 50.12 & 3.763 & 73.31 & -0.1684 \\ 
\hline
 5 & 63.10 & 1.258 & 49.89 & 0.01683 \\ 
\hline
 6 & 79.43 & -1.73 & 63.22 & -0.03198 \\ 
\hline
 7 & 100.00 & -1.422 & 46.63 & 0.05837 \\ 
\hline
 8 & 125.89 & -2.652 & 51.95 & -0.03582 \\ 
\hline
 9 & 158.49 & -2.4 & 57.28 & -0.05945 \\ 
\hline
10 & 199.53 & 0.4094 & 50.55 & -0.07848 \\ 
\hline
11 & 251.19 & 1.224 & 90.82 & -0.2405 \\ 
\hline
12 & 316.23 & 6.025 & 175.4 & -0.02752 \\ 
\hline
13 & 398.11 & 7.085 & 156.2 & -0.08729 \\ 
\hline
14 & 501.19 & 13.61 & 214.9 & -0.04846 \\ 
\hline
15 & 630.96 & 18.01 & 335.7 & 0.3702 \\ 
\hline
16 & 794.33 & 16.52 & 290.7 & 0.2108 \\ 
\hline
17 & 1000.00 & 14.64 & 236 & 0.1101 \\ 
\hline
18 & 1258.93 & 15.34 & 262.9 & -0.06771 \\ 
\hline
19 & 1584.89 & 12.5 & 198.7 & -0.2121 \\ 
\hline
20 & 1995.26 & 6.824 & 75.29 & 0.2415 \\ 
\hline
21 & 2511.89 & 5.671 & 53.68 & 0.2641 \\ 
\hline
22 & 3162.28 & 2.741 & 18.22 & 0.2656 \\ 
\hline
23 & 3981.07 & -0.166 & 9.568 & 0.2064 \\ 
\hline
24 & 5011.87 & -1.723 & 10.25 & 0.5951 \\ 
\hline
25 & 6309.57 & -2.282 & 13.73 & 0.6798 \\ 
\hline
26 & 7943.28 & -3.855 & 31.98 & 0.569 \\ 
\hline


==> ana_eval_gt_partic_results_combined_Phase3_TR_P3S_DRR_dB_18dB_SNR_All_Noises_sub_Velocity_cite_bias_sub.tex <==
 1 & 25.12 & 5.006 & 45.61 & -0.2541 \\ 
\hline
 2 & 31.62 & 5.454 & 46.52 & -0.1827 \\ 
\hline
 3 & 39.81 & 4.101 & 29.46 & 0.3129 \\ 
\hline
 4 & 50.12 & 3.332 & 29.53 & -0.3698 \\ 
\hline
 5 & 63.10 & 1.836 & 24.23 & -0.05317 \\ 
\hline
 6 & 79.43 & 1.782 & 26.4 & 0.1032 \\ 
\hline
 7 & 100.00 & 2.576 & 36.96 & 0.05147 \\ 
\hline
 8 & 125.89 & 4.309 & 36.71 & 0.1734 \\ 
\hline
 9 & 158.49 & 3.961 & 27.38 & 0.3398 \\ 
\hline
10 & 199.53 & 3.604 & 23.12 & 0.4239 \\ 
\hline
11 & 251.19 & 2.113 & 11.72 & 0.4645 \\ 
\hline
12 & 316.23 & 2.751 & 15.66 & 0.1251 \\ 
\hline
13 & 398.11 & 1.728 & 12 & 0.5963 \\ 
\hline
14 & 501.19 & 2.122 & 14.69 & 0.3958 \\ 
\hline
15 & 630.96 & 1.738 & 10.34 & 0.7411 \\ 
\hline
16 & 794.33 & -0.6083 & 7.401 & 0.6844 \\ 
\hline
17 & 1000.00 & 0.4545 & 7.015 & 0.555 \\ 
\hline
18 & 1258.93 & 1.167 & 7.763 & 0.5749 \\ 
\hline
19 & 1584.89 & -0.7357 & 9.062 & 0.1949 \\ 
\hline
20 & 1995.26 & -0.4119 & 6.931 & 0.5671 \\ 
\hline
21 & 2511.89 & -0.1258 & 5.229 & 0.4914 \\ 
\hline
22 & 3162.28 & -2.189 & 15.73 & 0.3221 \\ 
\hline


==> ana_eval_gt_partic_results_combined_Phase3_TR_P3S_T60_Perc_-1dB_SNR_All_Noises_sub_Frequency-dependent-RTE_cite_bias_sub.tex <==
 1 & 25.12 & -0.5347 & 2.914 & 0.126 \\ 
\hline
 2 & 31.62 & -0.06869 & 0.5554 & 0.02342 \\ 
\hline
 3 & 39.81 & 0.3829 & 0.5789 & 0.1708 \\ 
\hline
 4 & 50.12 & 0.3655 & 0.4964 & 0.06336 \\ 
\hline
 5 & 63.10 & 0.4307 & 0.5133 & 0.000547 \\ 
\hline
 6 & 79.43 & 0.3488 & 0.3137 & -0.09614 \\ 
\hline
 7 & 100.00 & 0.4941 & 0.3316 & 0.1043 \\ 
\hline
 8 & 125.89 & 0.3702 & 0.1897 & 0.4477 \\ 
\hline
 9 & 158.49 & 0.3033 & 0.1647 & 0.1927 \\ 
\hline
10 & 199.53 & 0.1761 & 0.1123 & 0.3598 \\ 
\hline
11 & 251.19 & 0.1163 & 0.1131 & 0.3251 \\ 
\hline
12 & 316.23 & 0.07613 & 0.09129 & 0.4367 \\ 
\hline
13 & 398.11 & 0.05576 & 0.09624 & 0.4649 \\ 
\hline
14 & 501.19 & 0.04185 & 0.1102 & 0.5055 \\ 
\hline
15 & 630.96 & 0.0323 & 0.1348 & 0.5339 \\ 
\hline
16 & 794.33 & 0.01266 & 0.1404 & 0.5578 \\ 
\hline
17 & 1000.00 & -0.01721 & 0.1472 & 0.5763 \\ 
\hline
18 & 1258.93 & -0.02465 & 0.1215 & 0.5892 \\ 
\hline
19 & 1584.89 & -0.0255 & 0.1101 & 0.5981 \\ 
\hline
20 & 1995.26 & -0.03887 & 0.1061 & 0.6038 \\ 
\hline
21 & 2511.89 & -0.07156 & 0.1078 & 0.589 \\ 
\hline
22 & 3162.28 & -0.04975 & 0.08151 & 0.5923 \\ 
\hline
23 & 3981.07 & -0.01704 & 0.05859 & 0.5959 \\ 
\hline
24 & 5011.87 & 0.01489 & 0.03508 & 0.5848 \\ 
\hline
25 & 6309.57 & 0.07755 & 0.02534 & 0.5997 \\ 
\hline
26 & 7943.28 & 0.06802 & 0.02342 & 0.6049 \\ 
\hline
27 & 10000.00 & 0.1189 & 0.03621 & 0.465 \\ 
\hline
28 & 12589.25 & 0.1989 & 0.05723 & 0.5912 \\ 
\hline
29 & 15848.93 & 0.265 & 0.09049 & 0.5806 \\ 
\hline
30 & 19952.62 & 0.3596 & 0.1552 & 0.1756 \\ 
\hline


==> ana_eval_gt_partic_results_combined_Phase3_TR_P3S_T60_Perc_12dB_SNR_All_Noises_sub_Frequency-dependent-RTE_cite_bias_sub.tex <==
 1 & 25.12 & -0.5247 & 2.908 & 0.1187 \\ 
\hline
 2 & 31.62 & -0.02764 & 0.5488 & 0.006539 \\ 
\hline
 3 & 39.81 & 0.4391 & 0.6089 & 0.1764 \\ 
\hline
 4 & 50.12 & 0.4197 & 0.5062 & 0.1053 \\ 
\hline
 5 & 63.10 & 0.4691 & 0.5255 & 0.01945 \\ 
\hline
 6 & 79.43 & 0.3639 & 0.3001 & -0.03721 \\ 
\hline
 7 & 100.00 & 0.4845 & 0.3048 & 0.1851 \\ 
\hline
 8 & 125.89 & 0.3392 & 0.1483 & 0.606 \\ 
\hline
 9 & 158.49 & 0.2568 & 0.121 & 0.3279 \\ 
\hline
10 & 199.53 & 0.12 & 0.06959 & 0.5279 \\ 
\hline
11 & 251.19 & 0.05571 & 0.07287 & 0.4944 \\ 
\hline
12 & 316.23 & 0.01471 & 0.05692 & 0.6058 \\ 
\hline
13 & 398.11 & -0.004296 & 0.06311 & 0.6365 \\ 
\hline
14 & 501.19 & -0.01566 & 0.07833 & 0.6743 \\ 
\hline
15 & 630.96 & -0.02217 & 0.1031 & 0.7038 \\ 
\hline
16 & 794.33 & -0.03873 & 0.112 & 0.7287 \\ 
\hline
17 & 1000.00 & -0.06569 & 0.1221 & 0.751 \\ 
\hline
18 & 1258.93 & -0.07052 & 0.1004 & 0.7634 \\ 
\hline
19 & 1584.89 & -0.0691 & 0.09103 & 0.7693 \\ 
\hline
20 & 1995.26 & -0.08052 & 0.08874 & 0.7753 \\ 
\hline
21 & 2511.89 & -0.1116 & 0.09345 & 0.7613 \\ 
\hline
22 & 3162.28 & -0.08842 & 0.06782 & 0.763 \\ 
\hline
23 & 3981.07 & -0.05462 & 0.04504 & 0.7635 \\ 
\hline
24 & 5011.87 & -0.0218 & 0.02263 & 0.7561 \\ 
\hline
25 & 6309.57 & 0.04158 & 0.01269 & 0.7709 \\ 
\hline
26 & 7943.28 & 0.03264 & 0.012 & 0.7687 \\ 
\hline
27 & 10000.00 & 0.08401 & 0.0231 & 0.6188 \\ 
\hline
28 & 12589.25 & 0.1644 & 0.04122 & 0.7206 \\ 
\hline
29 & 15848.93 & 0.2308 & 0.07245 & 0.6204 \\ 
\hline
30 & 19952.62 & 0.3256 & 0.1329 & 0.07444 \\ 
\hline


==> ana_eval_gt_partic_results_combined_Phase3_TR_P3S_T60_Perc_18dB_SNR_All_Noises_sub_Frequency-dependent-RTE_cite_bias_sub.tex <==
 1 & 25.12 & -0.4999 & 2.88 & 0.123 \\ 
\hline
 2 & 31.62 & 0.01326 & 0.5446 & -0.003468 \\ 
\hline
 3 & 39.81 & 0.4887 & 0.6378 & 0.1871 \\ 
\hline
 4 & 50.12 & 0.4699 & 0.5383 & 0.09536 \\ 
\hline
 5 & 63.10 & 0.5133 & 0.5619 & -0.007577 \\ 
\hline
 6 & 79.43 & 0.3982 & 0.3225 & -0.0849 \\ 
\hline
 7 & 100.00 & 0.5079 & 0.3254 & 0.1511 \\ 
\hline
 8 & 125.89 & 0.3528 & 0.1542 & 0.6326 \\ 
\hline
 9 & 158.49 & 0.2629 & 0.1223 & 0.3427 \\ 
\hline
10 & 199.53 & 0.121 & 0.06725 & 0.5485 \\ 
\hline
11 & 251.19 & 0.05378 & 0.06904 & 0.52 \\ 
\hline
12 & 316.23 & 0.0113 & 0.05326 & 0.6307 \\ 
\hline
13 & 398.11 & -0.00822 & 0.05796 & 0.6695 \\ 
\hline
14 & 501.19 & -0.01955 & 0.0726 & 0.7079 \\ 
\hline
15 & 630.96 & -0.02575 & 0.09706 & 0.7362 \\ 
\hline
16 & 794.33 & -0.04187 & 0.1051 & 0.7667 \\ 
\hline
17 & 1000.00 & -0.06837 & 0.1148 & 0.7907 \\ 
\hline
18 & 1258.93 & -0.07273 & 0.09344 & 0.8057 \\ 
\hline
19 & 1584.89 & -0.07086 & 0.08434 & 0.812 \\ 
\hline
20 & 1995.26 & -0.08187 & 0.08201 & 0.8191 \\ 
\hline
21 & 2511.89 & -0.1126 & 0.08674 & 0.8061 \\ 
\hline
22 & 3162.28 & -0.08908 & 0.06187 & 0.8081 \\ 
\hline
23 & 3981.07 & -0.05499 & 0.04 & 0.8086 \\ 
\hline
24 & 5011.87 & -0.02192 & 0.01909 & 0.8021 \\ 
\hline
25 & 6309.57 & 0.04168 & 0.01098 & 0.8167 \\ 
\hline
26 & 7943.28 & 0.03293 & 0.01032 & 0.8154 \\ 
\hline
27 & 10000.00 & 0.08446 & 0.02249 & 0.6619 \\ 
\hline
28 & 12589.25 & 0.165 & 0.04156 & 0.7611 \\ 
\hline
29 & 15848.93 & 0.2315 & 0.0739 & 0.6405 \\ 
\hline
30 & 19952.62 & 0.3264 & 0.1353 & 0.05742 \\ 
\hline

